The first nova eruption in a novalike variable: YZ Ret as seen in X-rays and gamma-rays

Peaking at 3.7 mag on 2020 July 11, YZ Ret was the second-brightest nova of the decade. The nova's moderate proximity (2.7 kpc from Gaia) provided an opportunity to explore its multi-wavelength properties in great detail. Here we report on YZ Ret as part of a long-term project to identify the physical mechanisms responsible for high-energy emission in classical novae. We use simultaneous Fermi/LAT and NuSTAR observations complemented by XMM-Newton X-ray grating spectroscopy to probe the physical parameters of the shocked ejecta and the nova-hosting white dwarf. The XMM-Newton observations revealed a super-soft X-ray emission which is dominated by emission lines of CV, CVI, NVI, NVII, and OVIII rather than a blackbody-like continuum, suggesting CO-composition of the white dwarf in a high-inclination binary system. Fermi/LAT detected YZ Ret for 15 days with the gamma-ray spectrum best described by a power law with an exponential cut-off at 1.9 +/-0.6 GeV. In stark contrast with theoretical predictions and in keeping with previous NuSTAR observations of Fermi-detected classical novae (V5855 Sgr and V906 Car), the 3.5-78 keV X-ray emission is found to be two orders of magnitude fainter than the GeV emission. The X-ray emission observed by NuSTAR is consistent with a single-temperature thermal plasma. We detect no non-thermal tail of the GeV emission expected to extend down to the NuSTAR band. NuSTAR observations continue to challenge theories of high-energy emission from shocks in novae.

==> Makefile <==
# Automated setup: try to find the tex file and recognize its format: PDF figure, BibTeX...
TEXFILE_BASENAME = $(shell ls *.tex | head -n1 | sed 's:.tex::g')

PDFTEX := $(shell cat *.tex | cut -f1 -d"%" | grep 'includegr' | grep --quiet -e '.pdf' -e '.png' && echo 'yes' )
BIBTEX := $(shell cat *.tex | cut -f1 -d"%" | grep --quiet 'bibliographystyle' && echo 'yes' )

MODIFY_BIBFILE_ULTRACOMPACT_REF := $(shell cat *.tex | cut -f1 -d"%" | grep --quiet -e 'bibliographystyle.mnras_shortlisthack' -e 'bibliographystyle.supershort_numbers_oneline' && echo 'yes' )

MNRAS_MANUSCRIPT_REQUIRING_BRITISH_SPELLING := $(shell cat *.tex | cut -f1 -d"%" | grep 'documentclass' | grep --quiet 'mnras' && echo 'yes' )

AAS_MANUSCRIPT_REQUIRING_US_SPELLING := $(shell cat *.tex | cut -f1 -d"%" | grep 'documentclass' | grep --quiet 'aastex' && echo 'yes' )

ANY_KNOWN_SOFTWARE_MENTIONED := $(shell cat *.tex | cut -f1 -d"%" | grep --quiet -e 'IRAF' -e 'MIDAS' -e 'AIPS' -e 'CASA' -e 'DS9' -e 'ds9' -e 'VaST' -e 'HEASoft' -e 'HEASOFT' -e 'HEAsoft' -e 'Fermitools' && echo 'yes' )

all: clean check_utf8 check_spell check_no_whitespace check_coma_instead_of_period check_extra_white_space try_to_find_duplicate_words shorten_journal_names_bib check_british_spelling check_us_spelling check_software_small_capitals $(TEXFILE_BASENAME).pdf

clean: 
	#rm -f $(TEXFILE_BASENAME).bbl  $(TEXFILE_BASENAME).pdf $(TEXFILE_BASENAME).ps $(TEXFILE_BASENAME).dvi $(TEXFILE_BASENAME).log $(TEXFILE_BASENAME).aux $(TEXFILE_BASENAME).blg DEADJOE *~ *.bak main_paper.pdf online_material.pdf $(TEXFILE_BASENAME).out $(TEXFILE_BASENAME).teximulated mn2e.bst_backup missfont.log *~
	# arXiv needs .bbl
	rm -f  $(TEXFILE_BASENAME).pdf $(TEXFILE_BASENAME).ps $(TEXFILE_BASENAME).dvi $(TEXFILE_BASENAME).log $(TEXFILE_BASENAME).aux $(TEXFILE_BASENAME).blg DEADJOE *~ *.bak main_paper.pdf online_material.pdf $(TEXFILE_BASENAME).out $(TEXFILE_BASENAME).teximulated mn2e.bst_backup missfont.log *~

check_utf8: $(TEXFILE_BASENAME).tex
	# Display any non-ASCII UTF8 characters higlighting them with color
	cat $(TEXFILE_BASENAME).tex | { grep --color=always '[^ -~]\+' && exit 1 || true; }
	# Check that the TeX file type is not Unicode
	file $(TEXFILE_BASENAME).tex | { grep Unicode && exit 1 || true; }

check_spell: $(TEXFILE_BASENAME).tex
	# Case-insensitive search
	cat $(TEXFILE_BASENAME).tex | sed 's:the A config::g' | sed 's:binary tree::g' | { grep --color=always --ignore-case -e 'compliment' -e 'complimented' -e 'ile up' -e 'ile~up' -e ' can will ' -e ' may can ' -e ' may will ' -e ' a the ' -e ' the a ' -e ' whited ' -e 'neutrons star' -e 'hotpot' -e ' rang ' -e 'has be seen' -e 'synchroton' -e 'hight' -e 'far from being settled' -e 'recourses' -e 'wile' -e 'will allows' -e ' tree ' -e ' an new' -e 'data is ' && exit 1 || true; }
	# Case-sensitive search
	cat $(TEXFILE_BASENAME).tex | sed 's:the A config::g' | { grep --color=always -e 'x-ray' && exit 1 || true; }
	#
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always 'countrate' && echo "SHOULD BE count rate" && exit 1 || true; }
	# Use \b to match on "word boundaries", which will make your search match on whole words only.
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always '\bgenue\b' && echo "SHOULD BE genuine" && exit 1 || true; }

check_no_whitespace: $(TEXFILE_BASENAME).tex
	#  cut -f1 -d"%" -- ignore everything after %
	#  sed -e 's/\[[^][]*\]//g' -- ignore everything between []
	#  sed -e 's/{[^{}]*}//g'   -- ignore everything between {}
	#
	# period
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | sed 's:R.A.::g' | sed 's:L.A.Cosmic::g' | sed 's:\\.M::g' | sed 's:Obs.ID::g' | sed 's:U.S.::g' | sed 's:H.E.S.S.::g' | sed 's:J.D.L.::g' | sed 's:K.V.S.::g' | sed 's:E.A.::g' | sed 's:Ras.Pi::g' | sed 's:Ph.D.::g' | sed 's:P.O.::g' | { grep --color=always -e '\.[A-Z]' && exit 1 || true; }
	# two periods
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep --color=always -e '\.\.' && exit 1 || true; }
	# coma periods
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep --color=always -e '\,\.' && exit 1 || true; }
	# some journal styles allow ".," combination: "e.g.,"
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep --color=always -e '\.\,' && exit 1 || true; }
	# two comas
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep --color=always -e '\,\,' && exit 1 || true; }
	#
	# White space between Fig. and ref
	cat $(TEXFILE_BASENAME).tex | { grep --color=always 'Fig\.\\ref' && echo "SHOULD BE Fig.~\\ref{}" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | { grep --color=always 'Fig\\ref' && echo "SHOULD BE Fig.~\\ref{}" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | { grep --color=always 'Figure\\ref' && echo "SHOULD BE Figure~\\ref{}" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | { grep --color=always 'Figure \\ref' && echo "SHOULD BE Figure~\\ref{}" && exit 1 || true; }
	# White space before \cite
	cat $(TEXFILE_BASENAME).tex | sed 's:\\protect\\citeauthoryear::g' | { grep --color=always '[a-z]\\cite' && echo "NO WHITE SPACE BEFORE \\cite" && exit 1 || true; }

check_extra_white_space: $(TEXFILE_BASENAME).tex
	cat $(TEXFILE_BASENAME).tex | { grep --color=always ' \.' && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | { grep --color=always ' \,' && exit 1 || true; }

check_coma_instead_of_period: $(TEXFILE_BASENAME).tex
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | grep -v -e 'Uni' -e 'Obs' -e 'Inst' | { grep --color=always -e '\,The' -e '\, The' && exit 1 || true; }

try_to_find_duplicate_words: $(TEXFILE_BASENAME).tex
	# Catch word repeats in one line
	# The old version that doesn't catch everything
	cat $(TEXFILE_BASENAME).tex | grep -v -E '[0-9]cm' | grep -v -E '[0-9]in' | grep -v -e '&' -e 'textwidth' -e 'includegraphicx' -e 'includegraphics' -e 'tabular' | { egrep "(\b[a-zA-Z]+) \1\b"  && exit 1 || true; }
	# The new experimental version
	#  sed -e 's/\[[^][]*\]//g' -- ignore everything between []
	#  sed -e 's/{[^{}]*}//g'   -- ignore everything between {}
	# mess 'caption{}' and 'captionbox{}' as we still want to check for repeated words in captions
	cat $(TEXFILE_BASENAME).tex | sed 's:\\it : :g' | sed 's:\\em : :g' | sed 's:\\bf : :g' | grep -v 'tabular' | sed 's:caption{::g' | sed 's:captionbox{::g' | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep -Ein --color  "\b(\w+)\b\s*\1\b" && exit 1 || true; }
	# Last-trench effort -- just grep for the most common repetition
	cat $(TEXFILE_BASENAME).tex | { grep --color=always ' the the ' && exit 1 || true; }
	#
	#
	# Checking for repeated words over linebreaks
	# We do not exclude comments, so line numbers will be correct
	cat $(TEXFILE_BASENAME).tex | sed 's:\\it : :g' | sed 's:\\em : :g' | sed 's:\\bf : :g' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | grep -v 'tabular' | sed 's:caption{::g' | sed 's:captionbox{::g' | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep -Ei --color  "\b(\w+)\b\s*\1\b" && exit 1 || true; }
	#  sed 's/%.*$//'    -- remove everything after %
	#  sed '/^[[:space:]]*$/d' -- remoove empty lines
	# The output line nubers may not be exact as we skip comment lines
	cat $(TEXFILE_BASENAME).tex | sed 's:\\it : :g' | sed 's:\\em : :g' | sed 's:\\bf : :g' | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | grep -v 'tabular' | sed 's:caption{::g' | sed 's:captionbox{::g' | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep -Ei --color  "\b(\w+)\b\s*\1\b" && exit 1 || true; }
	
# This hack will modify the .bib file replacing some long journal names if we are using mnras_shortlisthack.bst style
shorten_journal_names_bib:
ifeq ($(MODIFY_BIBFILE_ULTRACOMPACT_REF),yes)
	# Modify .bib
	echo "I WILL RUIN THE BIBFILE"
	echo $(MODIFY_BIBFILE_ULTRACOMPACT_REF)
	# If the bibfile looks unmodified, save a backup copy
	cat $(TEXFILE_BASENAME).bib | { grep -e '{ATel}' -e '{RNAAS}' -e '{AN}' || cp -v $(TEXFILE_BASENAME).bib $(TEXFILE_BASENAME).bib_backup_long_journal_names ; }
	# Do the actual modification
	cat $(TEXFILE_BASENAME).bib | sed 's:{The Astronomer.s Telegram}:{ATel}:g' | sed 's:{Research Notes of the American Astronomical Society}:{RNAAS}:g' | sed 's:{Astronomische Nachrichten}:{AN}:g' > $(TEXFILE_BASENAME).bib_tmp && mv -v $(TEXFILE_BASENAME).bib_tmp $(TEXFILE_BASENAME).bib
else
	# Nothing to do
	echo "KEEP THE ORIGINAL BIBFILE"
	echo $(MODIFY_BIBFILE_ULTRACOMPACT_REF)
endif

check_british_spelling:
ifeq ($(MNRAS_MANUSCRIPT_REQUIRING_BRITISH_SPELLING),yes)
	# Check for British spelling
	# MNRAS style guide https://academic.oup.com/mnras/pages/General_Instructions#6%20Style%20guide
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -v '$^{' | grep -v '\\center' | { grep --color=always 'centered' && echo "SHOULD BE centred" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -v '$^{' | grep -v '\\center' | { grep --color=always 'center' && echo "SHOULD BE centre" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'sulfur' && echo "SHOULD BE sulphur" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'labeled' && echo "SHOULD BE labelled" && exit 1 || true; }
	#
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'analyze' && echo "SHOULD BE analyse" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'parametrise' && echo "SHOULD BE parametrize" && exit 1 || true; }
	#
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'acknowledgments' && echo "SHOULD BE acknowledgements" && exit 1 || true; }
	#
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'artifact' && echo "SHOULD BE artefact" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'best-fit ' && echo "SHOULD BE best-fitting" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'disk' && echo "SHOULD BE disc" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'halos' && echo "SHOULD BE haloes" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'hot-spot' && echo "SHOULD BE hotspot" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'nonlinear' && echo "SHOULD BE non-linear" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case ' onto ' && echo "SHOULD BE on to" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'timescale' && echo "SHOULD BE time-scale" && exit 1 || true; }
	#
	# random collection of words
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'color' && echo "SHOULD BE colour" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'flavor' && echo "SHOULD BE flavour" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'humor' && echo "SHOULD BE humour" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -v '$^{' | { grep --color=always 'labor' && echo "SHOULD BE labour" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'neighbor' && echo "SHOULD BE neighbour" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'paralyze' && echo "SHOULD BE paralyse" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed 's:talogue::g' | { grep --color=always --ignore-case 'catalog' && echo "SHOULD BE catalogue" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'analog' && echo "SHOULD BE analogue" && exit 1 || true; }
	#
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'modeling' && echo "SHOULD BE modelling" && exit 1 || true; }
	# Other MNRAS things
	cat $(TEXFILE_BASENAME).tex | { grep --color=always --ignore-case '\\%' && echo "SHOULD BE per cent" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case -e '~sec ' -e ' sec ' -e '\\,sec' && echo "SHOULD BE s" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'e\.g\.\,' && echo "SHOULD BE e.g." && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'i\.e\.\,' && echo "SHOULD BE i.e." && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case -e 'cf\.\,' -e ' cf ' && echo "SHOULD BE cf." && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case ' etc ' && echo "SHOULD BE etc." && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case '``' && echo "SHOULD BE \`" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case "''" && echo "SHOULD BE \'" && exit 1 || true; }
else
	# Nothing to do
	echo "THIS DOES NOT LOOK LIKE A MNRAS MANUSCRIPT - NOT ENFORCING BRITISH SPELLING"
	echo $(MNRAS_MANUSCRIPT_REQUIRING_BRITISH_SPELLING)
endif

check_us_spelling:
ifeq ($(AAS_MANUSCRIPT_REQUIRING_US_SPELLING),yes)
	# Check for US spelling
	# AAS style guide https://journals.aas.org/aas-style-guide/
	# they also suggest follow The Chicago Manual of Style https://www.chicagomanualofstyle.org/home.html
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -v '$^{' | grep -v '\\center' | { grep --color=always 'centered' && echo "SHOULD BE centred" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -v '$^{' | grep -v '\\center' | { grep --color=always 'centred' && echo "SHOULD BE centered" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -v '$^{' | grep -v '\\center' | { grep --color=always 'center' && echo "SHOULD BE centre" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -v '$^{' | grep -v '\\center' | { grep --color=always 'centre' && echo "SHOULD BE center" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'sulfur' && echo "SHOULD BE sulphur" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'sulphur' && echo "SHOULD BE sulfur" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'labeled' && echo "SHOULD BE labelled" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'labelled' && echo "SHOULD BE labeled" && exit 1 || true; }
	#
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'analyze' && echo "SHOULD BE analyse" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'analyse' && echo "SHOULD BE analyze" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'parametrise' && echo "SHOULD BE parametrize" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'parametrize' && echo "SHOULD BE parametrise" && exit 1 || true; }
	# Yes, acknowledgements
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'acknowledgments' && echo "SHOULD BE acknowledgements" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'acknowledgements' && echo "SHOULD BE acknowledgments" && exit 1 || true; }
	#
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'artifact' && echo "SHOULD BE artefact" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'artefact' && echo "SHOULD BE artifact" && exit 1 || true; }
	# Yes, best-fitting seems to be OK at AAS
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'best-fit ' && echo "SHOULD BE best-fitting" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'best-fitting ' && echo "SHOULD BE best-fit" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'disk' && echo "SHOULD BE disc" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case -e ' disc\,' -e ' disc\.' -e 'disc$$' -e 'disc ' && echo "SHOULD BE disk" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'halos' && echo "SHOULD BE haloes" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'haloes' && echo "SHOULD BE halos" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'hot-spot' && echo "SHOULD BE hotspot" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'nonlinear' && echo "SHOULD BE non-linear" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case ' onto ' && echo "SHOULD BE on to" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case ' on to ' && echo "SHOULD BE onto" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'time-scale' && echo "SHOULD BE timescale" && exit 1 || true; }
	#
	# random collection of words
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'color' && echo "SHOULD BE colour" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'colour' && echo "SHOULD BE color" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'flavor' && echo "SHOULD BE flavour" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'flavour' && echo "SHOULD BE flavor" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'humor' && echo "SHOULD BE humour" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'humour' && echo "SHOULD BE humor" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -v '$^{' | { grep --color=always 'labor' && echo "SHOULD BE labour" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -v '$^{' | { grep --color=always 'labour' && echo "SHOULD BE labor" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'neighbor' && echo "SHOULD BE neighbour" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'neighbour' && echo "SHOULD BE neighbor" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'paralyze' && echo "SHOULD BE paralyse" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'paralyse' && echo "SHOULD BE paralyze" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed 's:talogue::g' | { grep --color=always --ignore-case 'catalog' && echo "SHOULD BE catalogue" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed 's:talogue::g' | { grep --color=always --ignore-case 'catalogue' && echo "SHOULD BE catalog" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'analog' && echo "SHOULD BE analogue" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'analogue' && echo "SHOULD BE analog" && exit 1 || true; }
	#
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'modeling' && echo "SHOULD BE modelling" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'modelling' && echo "SHOULD BE modeling" && exit 1 || true; }
	# Other AAS things
	#cat $(TEXFILE_BASENAME).tex | { grep --color=always --ignore-case '\\%' && echo "SHOULD BE per cent" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case -e '~sec ' -e ' sec ' -e '\\,sec' && echo "SHOULD BE s" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'e\.g\. ' && echo "SHOULD BE e.g.," && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'e\.g\.\]' && echo "SHOULD BE e.g.," && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'i\.e\. ' && echo "SHOULD BE i.e.," && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case -e 'cf\.\,' -e ' cf ' && echo "SHOULD BE cf." && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case ' etc ' && echo "SHOULD BE etc." && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case ' `[a-zA-Z]' && echo "SHOULD BE \`\`" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case "[a-zA-Z]' " && echo "SHOULD BE \'\'" && exit 1 || true; }
	# super AAS-specific
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always 'Fig\.' && echo "SHOULD BE Figure" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always 'Sec\.' && echo "SHOULD BE Section" && exit 1 || true; }
	#
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always 'errorbar' && echo "SHOULD BE error bar" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always 'free-fall' && echo "SHOULD BE freefall" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always 'free fall' && echo "SHOULD BE freefall" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always 'free~fall' && echo "SHOULD BE freefall" && exit 1 || true; }
else
	# Nothing to do
	echo "THIS DOES NOT LOOK LIKE AN AAS MANUSCRIPT - NOT ENFORCING US SPELLING"
	echo $(AAS_MANUSCRIPT_REQUIRING_US_SPELLING)
endif

check_software_small_capitals:
ifeq ($(ANY_KNOWN_SOFTWARE_MENTIONED),yes)
	# Check that \textsc is used in the text
	echo "CHECK IF \\textsc{SoftWare} IS USED"
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep '\\textsc'
else
	# Nothing to do
	echo "NO KNOWN SOFTWARE NAMES RECOGNIZED"
	echo $(ANY_KNOWN_SOFTWARE_MENTIONED)
endif

$(TEXFILE_BASENAME).pdf: $(TEXFILE_BASENAME).tex
ifeq ($(PDFTEX),yes)
	# pdflatex
	echo "YES PDF"
	echo $(PDFTEX)
ifeq ($(BIBTEX),yes)
	echo "YES BibTeX"
	echo $(BIBTEX)
	# This works with .pdf/.png figures
	pdflatex $(TEXFILE_BASENAME).tex && pdflatex $(TEXFILE_BASENAME).tex && bibtex $(TEXFILE_BASENAME) && pdflatex $(TEXFILE_BASENAME).tex && pdflatex $(TEXFILE_BASENAME).tex && texcount -v3 -merge -incbib -dir -sub=none -utf8 -sum $(TEXFILE_BASENAME).tex && okular $(TEXFILE_BASENAME).pdf
else
	echo "NO BibTeX"
	echo $(BIBTEX)
	# No BibTeX, .pdf/.png figures
	pdflatex $(TEXFILE_BASENAME).tex && pdflatex $(TEXFILE_BASENAME).tex && texcount -v3 -merge -incbib -dir -sub=none -utf8 -sum $(TEXFILE_BASENAME).tex && okular $(TEXFILE_BASENAME).pdf
endif

else
	# latex
	echo "NO PDF  "
	echo $(PDFTEX)
ifeq ($(BIBTEX),yes)
	echo "YES BibTeX"
	echo $(BIBTEX)
	# BibTeX and .eps figures (the right way)
	latex $(TEXFILE_BASENAME).tex && latex $(TEXFILE_BASENAME).tex && bibtex $(TEXFILE_BASENAME) && latex $(TEXFILE_BASENAME).tex && { latex $(TEXFILE_BASENAME).tex 2>&1 | grep --color=always 'undefined on input line' && exit 1 || true; } && dvips -o $(TEXFILE_BASENAME).ps $(TEXFILE_BASENAME).dvi && ps2pdf $(TEXFILE_BASENAME).ps && texcount -v3 -merge -incbib -dir -sub=none -utf8 -sum $(TEXFILE_BASENAME).tex && okular $(TEXFILE_BASENAME).pdf
else
	echo "NO BibTeX"
	echo $(BIBTEX)	
	# This works with .eps figures or when \usepackage[demo]{graphicx} is activated
	latex $(TEXFILE_BASENAME).tex && latex $(TEXFILE_BASENAME).tex && dvips -o $(TEXFILE_BASENAME).ps $(TEXFILE_BASENAME).dvi && ps2pdf $(TEXFILE_BASENAME).ps && texcount -v3 -merge -incbib -dir -sub=none -utf8 -sum $(TEXFILE_BASENAME).tex && okular $(TEXFILE_BASENAME).pdf
endif

endif
	
